From Play to Policy: Conditional Behavior Generation from Uncurated Robot Data

While large-scale sequence modeling from offline data has led to impressive performance gains in natural language and image generation, directly translating such ideas to robotics has been challenging. One critical reason for this is that uncurated robot demonstration data, i.e. play data, collected from non-expert human demonstrators are often noisy, diverse, and distributionally multi-modal. This makes extracting useful, task-centric behaviors from such data a difficult generative modeling problem. In this work, we present Conditional Behavior Transformers (C-BeT), a method that combines the multi-modal generation ability of Behavior Transformer with future-conditioned goal specification. On a suite of simulated benchmark tasks, we find that C-BeT improves upon prior state-of-the-art work in learning from play data by an average of 45.7%. Further, we demonstrate for the first time that useful task-centric behaviors can be learned on a real-world robot purely from play data without any task labels or reward information. Robot videos are best viewed on our project website: https://play-to-policy.github.io

==> repro_statement.tex <==
\section*{Reproducibility Statement}
As a part of our commitment to reproducibility, we plan to release all our code, data, and roll-out videos on the project website, \website.

We have already referred to the codebases that we build upon in Section~\ref{sec:app:hparams}, and included the hyperparameters used to train the models in our paper.
Finally, our simulated experiments are built on free environments and thus our experiments should be easily replicable.
